Commonsense-augmented Memory Construction and Management in Long-term Conversations via Context-aware Persona Refinement

Memorizing and utilizing speakers' personas is a common practice for response generation in long-term conversations. Yet, human-authored datasets often provide uninformative persona sentences that hinder response quality. This paper presents a novel framework that leverages commonsense-based persona expansion to address such issues in long-term conversation. While prior work focuses on not producing personas that contradict others, we focus on transforming contradictory personas into sentences that contain rich speaker information, by refining them based on their contextual backgrounds with designed strategies. As the pioneer of persona expansion in multi-session settings, our framework facilitates better response generation via human-like persona refinement. The supplementary video of our work is available at https://caffeine-15bbf.web.app/.

==> tables/RG_example.tex <==
\begin{table*}
\small
\centering
% \resizebox{\linewidth}{!}{
\begin{tabular}{cccccc}
\toprule
\multicolumn{6}{c}{\textbf{Dialogue Context}} \\
\multicolumn{6}{c} A: Do you know where to get a copy of the The Fugitive movies? \\
\multicolumn{6}{c} B: Sure! if you go to justwatch.com it will tell you where to buy a digital copy or you can go to walmart.com or amazon.  How's your Spanish learning going? \\
\multicolumn{6}{c} A: Perfect, thank you! I will look at all those places. I am still learning, and it is slow but I am trying! \\
\midrule
\multicolumn{6}{c}{\textbf{Persona Sentences}} \\ 
\multicolumn{2}{c}{Gold} & \multicolumn{2}{c}{Comet} & \multicolumn{2}{c}{Comet + Ours} \\ 
\cmidrule(lr){1-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6}
\multicolumn{2}{c}{I am trying to learn Spanish better.} & \multicolumn{2}{c}{I am trying to learn Spanish better.} & \multicolumn{2}{c}{I am trying to learn Spanish better.} \\  
\multicolumn{2}{c}{I'm learning Spanish.} & \multicolumn{2}{c}{I'm learning Spanish.} & \multicolumn{2}{c}{I am trying to learn Spanish better by watching shows and movies with Spanish subtitles.} \\  
\multicolumn{2}{c}{The Fugitive is my all time favorite movie.} & \multicolumn{2}{c}{The Fugitive is my all time favorite movie.} & \multicolumn{2}{c}{The Fugitive is my all time favorite movie.} \\  
\multicolumn{2}{c}{My Spanish language progress not much I'd expect.} & \multicolumn{2}{c}{I want to learn Spanish.} & \multicolumn{2}{c}{I'm learning Spanish.} \\  
\multicolumn{2}{c}{I like to speak in spanish.} & \multicolumn{2}{c}{I need to learn Spanish.} & \multicolumn{2}{c}{I am learning Spanish by watching movies.} \\  
\multicolumn{2}{c}{I like to watch that movie.} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{I need to read books to learn Spanish better.} \\  
\multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{I need to go to the library to learn Spanish, and my girlfriend might be interested in learning too.} \\  
\midrule 
\multicolumn{6}{c}{\textbf{Response Generation}} \\ 
\multicolumn{2}{c}{Gold} & \multicolumn{2}{c}{Comet} & \multicolumn{2}{c}{Comet + Ours} \\ 
\cmidrule(lr){1-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6}
\multicolumn{2}{c}{That's great to hear! Learning a new language can be challenging, but don't give up. Maybe try reading some Spanish plays to help improve your language skills.} & \multicolumn{2}{c}{That's great to hear! Learning a new language can take time, but as long as you're putting in the effort, you'll make progress. Keep it up!} & \multicolumn{2}{c}{That's great to hear! Learning a new language can take time, but as long as you're putting in the effort, you'll get there. Have you tried watching any Spanish movies with subtitles to practice?} \\
\bottomrule
\end{tabular}
% }
\caption{Response Generation Example}
\end{table*}


==> tables/RG_example_orig.tex <==
\begin{table*}
\small
\centering
\begin{tabular}{cccccc}
\toprule
\multicolumn{1}{c}{\multirow{4}{*}{\textbf{Dialogue Context}}} & \multicolumn{5}{c}{A: Hi} \\ 
\multicolumn{1}{c}{} & \multicolumn{5}{c}{B: Hello} \\ 
\multicolumn{1}{c}{} & \multicolumn{5}{c}{A: Hi} \\ 
\midrule
\multicolumn{6}{c}{\textbf{Persona Sentences}} \\ 
\multicolumn{2}{c}{Gold} & \multicolumn{2}{c}{Comet} & \multicolumn{2}{c}{Comet + Ours} \\ 
\cmidrule(lr){1-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6}
\multicolumn{2}{c}{I like vegetables} & \multicolumn{2}{c}{I like vegetables} & \multicolumn{2}{c}{I like vegetables} \\  
\multicolumn{2}{c}{I like vegetables} & \multicolumn{2}{c}{I like vegetables} & \multicolumn{2}{c}{I like vegetables} \\  
\multicolumn{2}{c}{} & \multicolumn{2}{c}{I like vegetables} & \multicolumn{2}{c}{I like vegetables} \\  
\multicolumn{2}{c}{} & \multicolumn{2}{c}{} & \multicolumn{2}{c}{I like vegetables} \\  
\midrule 
\multicolumn{6}{c}{\textbf{Response Generation}} \\ 
\multicolumn{2}{c}{Gold} & \multicolumn{2}{c}{Comet} & \multicolumn{2}{c}{Comet + Ours} \\ 
\cmidrule(lr){1-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6}
\multicolumn{2}{c}{Wow, Good} & \multicolumn{2}{c}{Wow, Great} & \multicolumn{2}{c}{Wow, Excellent} \\
\bottomrule
\end{tabular}
\caption{Response Generation Example}
\end{table*}

==> tables/human_eval_table.tex <==
\begin{table*}
\small
\centering
\begin{tabular}{lcccccccccc}
\toprule
\textit{Human Eval} &

  \multicolumn{2}{c}{\textbf{Engagingness}} &
  \multicolumn{2}{c}{\textbf{Humanlikeness}} &
  \multicolumn{2}{c}{\textbf{Consistency}} &
  \multicolumn{2}{c}{\textbf{Specificity}} &
  \multicolumn{2}{c}{\textbf{Memory-coherence}}
  \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(l){8-9} \cmidrule(l){10-11} 
\textbf{Model} &
  \textbf{win (\%)} &
  \textbf{lose (\%)} &
  \textbf{win (\%)} &
  \textbf{lose (\%)} &
  \textbf{win (\%)} &
  \textbf{lose (\%)} &
  \textbf{win (\%)} &
  \textbf{lose (\%)} &
  \textbf{win (\%)} &
  \textbf{lose (\%)} 
  \\ \midrule
Gold  & - & - & - & - & - & - & - & - & - & - \\
Comet & - & - & - & - & - & - & - & - & - & - \\
Comet + Ours & - & - & - & - & - & - & - & - & - & - \\ \bottomrule
\end{tabular}
\caption{Human eval table}
\end{table*}

% version 2 (?)
\begin{table*}
\small
\centering
\begin{tabular}{@{}lccccc@{}}
\toprule
\textbf{Model} &
\textbf{Engagingness} &
\textbf{Humanlikeness} &
\textbf{Consistency} &
\textbf{Specificity} &
\textbf{Memory-coherence}
\\ \midrule
Gold  & - & - & - & - & - \\
Comet & - & - & - & - & - \\
Comet + Ours & - & - & - & - & - \\
\bottomrule
\end{tabular}
\caption{Human eval table 2}
\end{table*}

==> tables/win_loss.tex <==
\begin{table*}
\small
\centering
\begin{tabular}{l|ccccccccccccc|c}
\hline CPX vs. COMET & \multicolumn{3}{|c}{ Desire (I want) } & \multicolumn{3}{c}{ Intent (I need) } & \multicolumn{3}{c}{ Emotion (I feel) } & \multicolumn{2}{c}{ Status (I am) } & \multicolumn{2}{c}{ Average } \\
\hline \multicolumn{1}{c}{ Metrics } & win & loss & $k$ & win & loss & $k$ & win & loss & $k$ & win & loss & $k$ & win & loss \\
\hline Engagement & $\mathbf{8 7 . 7}$ & 12.3 & 0.61 & $\mathbf{8 5 . 7}$ & 14.3 & 0.66 & $\mathbf{9 1 . 2}$ & 5.7 & 0.68 & $\mathbf{8 2 . 3}$ & 17.7 & 0.63 & $\mathbf{8 6 . 4}$ & 13.0 \\
Diversity & $\mathbf{9 0 . 3}$ & 9.7 & 0.72 & $\mathbf{8 9 . 0}$ & 5.7 & 0.68 & $\mathbf{9 2 . 7}$ & 4.3 & 0.70 & $\mathbf{9 4 . 3}$ & 4.2 & 0.69 & $\mathbf{9 1 . 6}$ & 6.0 \\
Relevance & $\mathbf{5 2 . 1}$ & 47.4 & 0.52 & $\mathbf{6 2 . 7}$ & 33.3 & 0.54 & 43.5 & $\mathbf{5 6 . 5}$ & 0.48 & 49.2 & $\mathbf{5 0 . 8}$ & 0.45 & $\mathbf{5 1 . 9}$ & 47.0 \\
\hline
\end{tabular}
\caption{}
\end{table*}
